"One Soy Latte for Daniel": Visual and Movement Communication of Intention from a Robot Waiter to a Group of Customers

Service robots are increasingly employed in the hospitality industry for delivering food orders in restaurants. However, in current practice the robot often arrives at a fixed location for each table when delivering orders to different patrons in the same dining group, thus requiring a human staff member or the customers themselves to identify and retrieve each order. This study investigates how to improve the robot's service behaviours to facilitate clear intention communication to a group of users, thus achieving accurate delivery and positive user experiences. Specifically, we conduct user studies (N=30) with a Temi service robot as a representative delivery robot currently adopted in restaurants. We investigated two factors in the robot's intent communication, namely visualisation and movement trajectories, and their influence on the objective and subjective interaction outcomes. A robot personalising its movement trajectory and stopping location in addition to displaying a visualisation of the order yields more accurate intent communication and successful order delivery, as well as more positive user perception towards the robot and its service. Our results also showed that individuals in a group have different interaction experiences.

==> old_results.tex <==
%old results
\subsection{Perception towards robot and interaction}
\begin{figure*}[tb]
    \centering
    \subfloat[][Anthropomorphism]{\includegraphics[width=0.3\linewidth]{figs/anthro.png}\label{fig:godspeed_anthro}}\\
    \subfloat[][Animacy]{\includegraphics[width=0.3\linewidth]{figs/anim.png}\label{fig:godspeed_anim}}\\
    \subfloat[][Likeability]{\includegraphics[width=0.3\linewidth]{figs/like.png}\label{fig:godspeed_like}}\\
    \subfloat[][Perceived Intelligence]{\includegraphics[width=0.3\linewidth]{figs/intel.png}\label{fig:godspeed_intel}}\\
    \subfloat[][Perceived Safety]{\includegraphics[width=0.3\linewidth]{figs/safe.png}\label{fig:godspeed_safe}}
     \caption{Rating differences in Godspeed questionnaire}
\label{fig:godspeed}
\end{figure*}

\begin{figure}[tb]
    \centering
    \subfloat[][Fluency]{\includegraphics[width=0.8\linewidth]{figs/fluen.png}\label{fig:fluen}}\\
    \subfloat[][Trust]{\includegraphics[width=0.8\linewidth]{figs/trust.png}\label{fig:trust}}\\
    \subfloat[][Working Alliance]{\includegraphics[width=0.8\linewidth]{figs/alli.png}\label{fig:alliance}}\\
    \subfloat[][Service Satisfaction]{\includegraphics[width=0.8\linewidth]{figs/satis.png}\label{fig:satisfy}}\\
    \subfloat[][Perceived Service Efficiency]{\includegraphics[width=0.8\linewidth]{figs/effec.png}\label{fig:effec}}
     \caption{Rating differences in interaction experience}
\label{fig:colab}
\end{figure}

\begin{figure}[tb]
    \centering
    \includegraphics[width=01\linewidth]{figs/anthro.png}
    \caption{Differences in anthropomorphism towards the robot: we found a statistically significant difference for customer type ($F(2,588) = 8.9361$, $p = 1.5028e-4$) and interaction between stopping type and customer type  ($F(2,588) = 3.5150$, $p = 0.0304$)}
\label{fig:anthro}
\end{figure}
\begin{figure}[tb]
    \centering
    \includegraphics[width=1\linewidth]{figs/anim.png}
    \caption{Differences in animacy towards the robot: we found a statistically significant difference for customer type ($F(2,588) = 9.0691$, $p = 1.3209e-4$) and interaction between stopping type and customer type  ($F(2,588) = 4.4811$, $p = 0.0117$)}
\label{fig:anim}
\end{figure}
\begin{figure}[tb]
    \centering
    \includegraphics[width=1\linewidth]{figs/like.png}
    \caption{Differences in likeability towards the robot: we found a statistically significant difference for customer type ($F(2,708) = 13.5167$, $p = 1.7341e-6$)}
\label{fig:like}
\end{figure}
\begin{figure}[tb]
    \centering
    \includegraphics[width=1\linewidth]{figs/intel.png}
    \caption{Differences in perceived intelligence towards the robot: we found a statistically significant difference for customer type ($F(2,588) = 15.9457$, $p = 1.8037e-7$)}
\label{fig:intel}
\end{figure}
\begin{figure}[tb]
    \centering
    \includegraphics[width=1\linewidth]{figs/safe.png}
    \caption{Differences in perceived safety: only customer type was statistically significant ($F(2,348) = 4.9590$, $p = 0.0075$)}
\label{fig:safe}
\end{figure}


\begin{figure}[tb]
    \centering
    \includegraphics[width=1\linewidth]{figs/fluen.png}
    \caption{Differences in fluency towards the robot: we found a statistically significant difference for customer type ($F(2,228) = 10.0779$, $p = 6.3972e-5$)}
\label{fig:fluen}
\end{figure}
\begin{figure}[tb]
    \centering
    \includegraphics[width=1\linewidth]{figs/trust.png}
    \caption{Differences in trust towards the robot: we found a statistically significant difference for customer type ($F(2,228) = 10.4581$, $p = 4.5134e-5$)}
\label{fig:trust}
\end{figure}
\begin{figure}[tb]
    \centering
    \includegraphics[width=1\linewidth]{figs/alli.png}
    \caption{Differences in working alliance towards the robot: we found a statistically significant difference for customer type ($F(2,348) = 9.5410$, $p = 9.2470e-5$), the interaction between stopping type and customer type  ($F(2,348) = 3.3020$, $p = 0.0380$) and the interaction between all three factors ($F(2,348) = 3.4704$, $p = 0.0322$)}
\label{fig:alli}
\end{figure}
\begin{figure}[tb]
    \centering
    \includegraphics[width=1\linewidth]{figs/satis.png}
    \caption{Differences in satisfaction towards the interaction: only indications and stopping type were significant.}
\label{fig:satis}
\end{figure}
\begin{figure}[tb]
    \centering
    \includegraphics[width=1\linewidth]{figs/effec.png}
    \caption{Differences in perceived efficiency towards the robot: we found a statistically significant difference for customer type ($F(2,108) = 5.8142$, $p = 0.0040$)}
\label{fig:effec}
\end{figure}

\begin{itemize}
    \item For anthropomorphism, we found a statistically significant difference for customer type ($F(2,588) = 8.9361$, $p = 1.5028e-4$) and interaction between stopping type and customer type  ($F(2,588) = 3.5150$, $p = 0.0304$). having the visualisations had a slightly higher mean rating than without visualisations. Personalised stopping as opposed to general stops also had slightly higher ratings. Customer type A gave the highest ratings whilst the lowest ratings were given by customer type C. The presence of indications, stopping type and customer type was statistically significant, as well as the joint significance of indications with stopping type and stopping type with customer type. The rest of the joint combinations were not statistically significant.
    \item For animacy, we found a statistically significant difference for customer type ($F(2,588) = 9.0691$, $p = 1.3209e-4$) and interaction between stopping type and customer type  ($F(2,588) = 4.4811$, $p = 0.0117$). having the visualisations had a slightly higher mean rating than without visualisations. Personalised stopping as opposed to general stops also had slightly higher ratings. Customer type A gave the highest ratings whilst the lowest ratings were given by customer type C. Indications were not statistically significant whilst stopping type and customer type were. For the joint combinations, indications with stopping type as well as stopping type with customer type were statistically significant whilst the rest are not.
    \item For likeability, we found a statistically significant difference for customer type ($F(2,708) = 13.5167$, $p = 1.7341e-6$). having the visualisations had a slightly higher mean rating than without visualisations. Personalised stopping as opposed to general stops also had slightly higher ratings. Customer type B gave the highest ratings whilst the lowest ratings were given by customer type C. The presence of indications, stopping type and customer type was statistically significant, as well as the joint significance of indications with stopping type. The rest of the joint combinations were not statistically significant.
    \item For intelligence, we found a statistically significant difference for customer type ($F(2,588) = 15.9457$, $p = 1.8037e-7$). having visualisations had a higher mean rating than without visualisations. Personalised stopping as opposed to general stops also had higher ratings. Customer type B gave the highest ratings whilst the lowest ratings were given by customer type C. The presence of indications, stopping type and customer type was statistically significant, as well as the joint significance of indications with stopping type. The other joint combinations were not statistically significant.
    \item For safety, only customer type was statistically significant ($F(2,348) = 4.9590$, $p = 0.0075$). having visualisations had a higher mean rating than without visualisations. Personalised stopping as opposed to general stops also had higher ratings. Customer type A gave the highest ratings whilst the lowest ratings were given by customer type C. Only indications and customer type were statistically significant while stopping type and all the combinations of the variables were not statistically significant.
\end{itemize}

\begin{itemize}
    \item For human-robot fluency, we found a statistically significant difference for customer type ($F(2,228) = 10.0779$, $p = 6.3972e-5$). having visualisations had a higher mean rating than without visualisations. Personalised stopping as opposed to general stops also had higher ratings. Customer type B gave the highest ratings whilst the lowest ratings were given by customer type C. The presence of indications, stopping type and customer type was statistically significant, as well as the joint significance of indications with stopping type. The rest of the joint combinations were not statistically significant.
    \item For trust in robot, we found a statistically significant difference for customer type ($F(2,228) = 10.4581$, $p = 4.5134e-5$). having visualisations had a higher mean rating than without visualisations. Personalised stopping as opposed to general stops also had higher ratings. Customer type B gave the highest ratings whilst the lowest ratings were given by customer type C. Indications, stopping type and customer type were statistically significant. However, all the combinations of the three variables were not statistically significant.
    \item For working alliance, we found a statistically significant difference for customer type ($F(2,348) = 9.5410$, $p = 9.2470e-5$), the interaction between stopping type and customer type  ($F(2,348) = 3.3020$, $p = 0.0380$) and the interaction between all three factors ($F(2,348) = 3.4704$, $p = 0.0322$). having visualisations had a higher mean rating than without visualisations. Personalised stopping as opposed to general stops also had higher ratings. Customer type B gave the highest ratings whilst the lowest ratings were given by customer type C. All variables as well as the joint combinations, except the combination of indications and customer type, were statistically significant.
    \item For perceived satisfaction, only indications and stopping type were significant. having visualisations had higher ratings than without visualisations. Personalised stopping as opposed to general stops also had higher ratings. Customer type A had the highest ratings whilst customer type C had the lowest ratings. While indications and stopping type are statistically significant, customer type and the joint combination of these variables are not statistically significant.
    \item For perceived efficiency, we found a statistically significant difference for customer type ($F(2,108) = 5.8142$, $p = 0.0040$). having visualisations had lower ratings than without visualisations. Personalised stopping as opposed to general stops had higher ratings. Customer type B had the highest ratings whilst customer type C had the lowest ratings. While indications and customer type are statistically significant, stopping type and the joint combination of these variables are not statistically significant.
\end{itemize}

\section{Results}
\subsection{Pre-study impressions}
\label{tab:godspeed_pre}
\begin{table}[tb]
\begin{tabular}{|l|r|r|}
\hline
GodSpeed item & Mean & Std\\
\hline
Anthropomorphism & 2.49 & 1.03\\
\hline
Animacy & 2.51 & 1.06\\
\hline
Likeability & 3.55 & 0.76\\
\hline
Intelligence & 3.18 & 0.97\\
\hline
Safety & 3.36 & 1.47\\
\hline
\end{tabular}
\end{table}

These were the initial ratings that participants gave of the robot before they were exposed to any of the conditions.
\subsection{Participant preferences}
\begin{table}[tb]
\begin{tabular}{|l|r|r|r|r|}
\hline
\multicolumn{1}{|c|}{\textbf{All groups}}  & \multicolumn{1}{l|}{General stop + no visual} & \multicolumn{1}{l|}{General stop + visual} & \multicolumn{1}{l|}{Personal stop + no visual} & \multicolumn{1}{l|}{Personal stop + visual} \\ \hline
Number of 1st preference                   & 4                                             & 8                                          & 0                                              & 18                                          \\ \hline
Number of 2nd preference                   & 4                                             & 16                                         & 3                                              & 7                                           \\ \hline
Number of 3rd preference                   & 9                                             & 4                                          & 13                                             & 4                                           \\ \hline
Number of 4th preference                   & 13                                            & 2                                          & 14                                             & 1                                           \\ \hline
                                           & \multicolumn{1}{l|}{}                         & \multicolumn{1}{l|}{}                      & \multicolumn{1}{l|}{}                          & \multicolumn{1}{l|}{}                       \\ \hline
\multicolumn{1}{|c|}{\textbf{All A group}} & \multicolumn{1}{l|}{General stop + no visual} & \multicolumn{1}{l|}{General stop + visual} & \multicolumn{1}{l|}{Personal stop + no visual} & \multicolumn{1}{l|}{Personal stop + visual} \\ \hline
Number of 1st preference                   & 1                                             & 2                                          & 0                                              & 7                                           \\ \hline
Number of 2nd preference                   & 1                                             & 7                                          & 1                                              & 1                                           \\ \hline
Number of 3rd preference                   & 3                                             & 1                                          & 5                                              & 1                                           \\ \hline
Number of 4th preference                   & 5                                             & 0                                          & 4                                              & 1                                           \\ \hline
                                           & \multicolumn{1}{l|}{}                         & \multicolumn{1}{l|}{}                      & \multicolumn{1}{l|}{}                          & \multicolumn{1}{l|}{}                       \\ \hline
\multicolumn{1}{|c|}{\textbf{All B group}} & \multicolumn{1}{l|}{General stop + no visual} & \multicolumn{1}{l|}{General stop + visual} & \multicolumn{1}{l|}{Personal stop + no visual} & \multicolumn{1}{l|}{Personal stop + visual} \\ \hline
Number of 1st preference                   & 3                                             & 3                                          & 0                                              & 4                                           \\ \hline
Number of 2nd preference                   & 1                                             & 5                                          & 0                                              & 4                                           \\ \hline
Number of 3rd preference                   & 4                                             & 0                                          & 4                                              & 2                                           \\ \hline
Number of 4th preference                   & 2                                             & 2                                          & 6                                              & 0                                           \\ \hline
                                           & \multicolumn{1}{l|}{}                         & \multicolumn{1}{l|}{}                      & \multicolumn{1}{l|}{}                          & \multicolumn{1}{l|}{}                       \\ \hline
\multicolumn{1}{|c|}{\textbf{All C group}} & \multicolumn{1}{l|}{General stop + no visual} & \multicolumn{1}{l|}{General stop + visual} & \multicolumn{1}{l|}{Personal stop + no visual} & \multicolumn{1}{l|}{Personal stop + visual} \\ \hline
Number of 1st preference                   & 0                                             & 3                                          & 0                                              & 7                                           \\ \hline
Number of 2nd preference                   & 2                                             & 4                                          & 2                                              & 2                                           \\ \hline
Number of 3rd preference                   & 2                                             & 3                                          & 4                                              & 1                                           \\ \hline
Number of 4th preference                   & 6                                             & 0                                          & 4                                              & 0                                           \\ \hline
\end{tabular}
\end{table}

Across all the groups personalised stops and visual indications had the most number of 1st preferences. General stops with visuals had the largest number of 2nd preferences whilst personal stops with no visualisations had the most number of 3rd and 4th preferences.

For participants who were customer A, the trend is similar with personal stops and visualisations having the most 1st preferences, and general stop with visuals having the most number of 2nd preferences. However, personal stops with no visuals had the most number of 3rd preferences whilst general stop with no visuals had the most number of 4th preferences.

For participants who were customer B, a similar trend with personal stops and visualisations having the most 1st preferences, and general stop with visuals having the most number of 2nd preferences. However, personal stops with no visuals had the most number of 3rd preferences tied with general stops with no visuals whilst personal stops with no visuals also had the most number of 4th preferences.

For participants who were customer C, once again it is a similar trend with personal stops and visualisations having the most 1st preferences, and general stop with visuals having the most number of 2nd preferences. However, while personal stops with no visuals had the most number of 3rd preferences, general stop with no visuals had the most number of 4th preferences.

\subsection{Means and variances}
\begin{table}[tb]
\caption{Anthropomorphism}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
          &          &   & \multicolumn{1}{r|}{Count} & \multicolumn{1}{r|}{Mean} & \multicolumn{1}{r|}{Variance} \\ \hline
No visual &          &   & 300                        & 2.7133333                 & 1.20851728                    \\ \hline
Visual    &          &   & 300                        & 2.96                      & 1.369632107                   \\ \hline
          & General  &   & 300                        & 2.7566667                 & 1.40212932                    \\ \hline
          & Personal &   & 300                        & 2.9166667                 & 1.193701226                   \\ \hline
          &          & A & 200                        & 3.015                     & 1.351532663                   \\ \hline
          &          & B & 200                        & 2.925                     & 1.094849246                   \\ \hline
          &          & C & 200                        & 2.57                      & 1.361909548                   \\ \hline
No visual & General  &   & 150                        & 2.7266667                 & 1.327472036                   \\ \hline
No visual & Personal &   & 150                        & 2.7                       & 1.097315436                   \\ \hline
Visual    & General  &   & 150                        & 2.7866667                 & 1.484384787                   \\ \hline
Visual    & Personal &   & 150                        & 3.1333333                 & 1.203579418                   \\ \hline
No visual &          & A & 100                        & 2.87                      & 1.245555556                   \\ \hline
No visual &          & B & 100                        & 2.87                      & 1.083939394                   \\ \hline
No visual &          & C & 100                        & 2.4                       & 1.171717172                   \\ \hline
Visual    &          & A & 100                        & 3.16                      & 1.428686869                   \\ \hline
Visual    &          & B & 100                        & 2.98                      & 1.110707071                   \\ \hline
Visual    &          & C & 100                        & 2.74                      & 1.507474747                   \\ \hline
          & General  & A & 100                        & 2.94                      & 1.309494949                   \\ \hline
          & General  & B & 100                        & 2.99                      & 1.282727273                   \\ \hline
          & General  & C & 100                        & 2.34                      & 1.378181818                   \\ \hline
          & Personal & A & 100                        & 3.09                      & 1.395858586                   \\ \hline
          & Personal & B & 100                        & 2.86                      & 0.909494949                   \\ \hline
          & Personal & C & 100                        & 2.8                       & 1.252525253                   \\ \hline
No visual & General  & A & 50                         & 2.86                      & 1.306530612                   \\ \hline
No visual & General  & B & 50                         & 3                         & 1.306122449                   \\ \hline
No visual & General  & C & 50                         & 2.32                      & 1.160816327                   \\ \hline
No visual & Personal & A & 50                         & 2.88                      & 1.209795918                   \\ \hline
No visual & Personal & B & 50                         & 2.74                      & 0.849387755                   \\ \hline
No visual & Personal & C & 50                         & 2.48                      & 1.193469388                   \\ \hline
Visual    & General  & A & 50                         & 3.02                      & 1.326122449                   \\ \hline
Visual    & General  & B & 50                         & 2.98                      & 1.285306122                   \\ \hline
Visual    & General  & C & 50                         & 2.36                      & 1.622857143                   \\ \hline
Visual    & Personal & A & 50                         & 3.3                       & 1.520408163                   \\ \hline
Visual    & Personal & B & 50                         & 2.98                      & 0.95877551                    \\ \hline
Visual    & Personal & C & 50                         & 3.12                      & 1.128163265                   \\ \hline
          &          &   & 600                        & 2.8366667                 & 1.302159154                   \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For anthropomorphism, having the visualisations had a slightly higher mean rating than without visualisations. Personalised stopping as opposed to general stops also had slightly higher ratings. Customer type A gave the highest ratings whilst the lowest ratings were given by customer type C.
\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\
\begin{table}[tb]
\caption{Animacy}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
          &          &   & \multicolumn{1}{r|}{Count} & \multicolumn{1}{r|}{Mean} & \multicolumn{1}{r|}{Variance} \\ \hline
No visual &          &   & 300                        & 2.83                      & 1.205117057                   \\ \hline
Visual    &          &   & 300                        & 2.9333333                 & 1.212931996                   \\ \hline
          & General  &   & 300                        & 2.7366667                 & 1.1912932                     \\ \hline
          & Personal &   & 300                        & 3.0266667                 & 1.189921962                   \\ \hline
          &          & A & 200                        & 3.03                      & 1.114673367                   \\ \hline
          &          & B & 200                        & 2.995                     & 1.090427136                   \\ \hline
          &          & C & 200                        & 2.62                      & 1.332261307                   \\ \hline
No visual & General  &   & 150                        & 2.7866667                 & 1.135391499                   \\ \hline
No visual & Personal &   & 150                        & 2.8733333                 & 1.279149888                   \\ \hline
Visual    & General  &   & 150                        & 2.6866667                 & 1.2501566                     \\ \hline
Visual    & Personal &   & 150                        & 3.18                      & 1.061342282                   \\ \hline
No visual &          & A & 100                        & 2.92                      & 1.145050505                   \\ \hline
No visual &          & B & 100                        & 3                         & 1.111111111                   \\ \hline
No visual &          & C & 100                        & 2.57                      & 1.277878788                   \\ \hline
Visual    &          & A & 100                        & 3.14                      & 1.071111111                   \\ \hline
Visual    &          & B & 100                        & 2.99                      & 1.080707071                   \\ \hline
Visual    &          & C & 100                        & 2.67                      & 1.395050505                   \\ \hline
          & General  & A & 100                        & 2.76                      & 0.871111111                   \\ \hline
          & General  & B & 100                        & 3.03                      & 1.261717172                   \\ \hline
          & General  & C & 100                        & 2.42                      & 1.276363636                   \\ \hline
          & Personal & A & 100                        & 3.3                       & 1.222222222                   \\ \hline
          & Personal & B & 100                        & 2.96                      & 0.927676768                   \\ \hline
          & Personal & C & 100                        & 2.82                      & 1.320808081                   \\ \hline
No visual & General  & A & 50                         & 2.82                      & 0.926122449                   \\ \hline
No visual & General  & B & 50                         & 3.06                      & 1.322857143                   \\ \hline
No visual & General  & C & 50                         & 2.48                      & 1.030204082                   \\ \hline
No visual & Personal & A & 50                         & 3.02                      & 1.366938776                   \\ \hline
No visual & Personal & B & 50                         & 2.94                      & 0.914693878                   \\ \hline
No visual & Personal & C & 50                         & 2.66                      & 1.535102041                   \\ \hline
Visual    & General  & A & 50                         & 2.7                       & 0.826530612                   \\ \hline
Visual    & General  & B & 50                         & 3                         & 1.224489796                   \\ \hline
Visual    & General  & C & 50                         & 2.36                      & 1.54122449                    \\ \hline
Visual    & Personal & A & 50                         & 3.58                      & 0.94244898                    \\ \hline
Visual    & Personal & B & 50                         & 2.98                      & 0.95877551                    \\ \hline
Visual    & Personal & C & 50                         & 2.98                      & 1.08122449                    \\ \hline
          &          &   & 600                        & 2.8816667                 & 1.209680022                   \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For animacy, having the visualisations had a slightly higher mean rating than without visualisations. Personalised stopping as opposed to general stops also had slightly higher ratings. Customer type A gave the highest ratings whilst the lowest ratings were given by customer type C.
\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\
\begin{table}[tb]
\caption{Likeability}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
          &          &   & \multicolumn{1}{r|}{Count} & \multicolumn{1}{r|}{Mean} & \multicolumn{1}{r|}{Variance} \\ \hline
No visual &          &   & 360                        & 3.241666667               & 1.309122563                   \\ \hline
Visual    &          &   & 360                        & 3.513888889               & 1.253288456                   \\ \hline
          & General  &   & 360                        & 3.186111111               & 1.427661715                   \\ \hline
          & Personal &   & 360                        & 3.569444444               & 1.098228103                   \\ \hline
          &          & A & 240                        & 3.325                     & 1.132426778                   \\ \hline
          &          & B & 240                        & 3.658333333               & 0.778172943                   \\ \hline
          &          & C & 240                        & 3.15                      & 1.860251046                   \\ \hline
No visual & General  &   & 180                        & 3.172222222               & 1.227157045                   \\ \hline
No visual & Personal &   & 180                        & 3.311111111               & 1.388702669                   \\ \hline
Visual    & General  &   & 180                        & 3.2                       & 1.63575419                    \\ \hline
Visual    & Personal &   & 180                        & 3.827777778               & 0.679671012                   \\ \hline
No visual &          & A & 120                        & 3.216666667               & 0.994677871                   \\ \hline
No visual &          & B & 120                        & 3.616666667               & 0.742577031                   \\ \hline
No visual &          & C & 120                        & 2.891666667               & 1.946148459                   \\ \hline
Visual    &          & A & 120                        & 3.433333333               & 1.256022409                   \\ \hline
Visual    &          & B & 120                        & 3.7                       & 0.816806723                   \\ \hline
Visual    &          & C & 120                        & 3.408333333               & 1.655392157                   \\ \hline
          & General  & A & 120                        & 3.05                      & 0.905042017                   \\ \hline
          & General  & B & 120                        & 3.583333333               & 1.018207283                   \\ \hline
          & General  & C & 120                        & 2.925                     & 2.137184874                   \\ \hline
          & Personal & A & 120                        & 3.6                       & 1.216806723                   \\ \hline
          & Personal & B & 120                        & 3.733333333               & 0.533333333                   \\ \hline
          & Personal & C & 120                        & 3.375                     & 1.496848739                   \\ \hline
No visual & General  & A & 60                         & 3.116666667               & 0.511581921                   \\ \hline
No visual & General  & B & 60                         & 3.616666667               & 1.087853107                   \\ \hline
No visual & General  & C & 60                         & 2.783333333               & 1.765819209                   \\ \hline
No visual & Personal & A & 60                         & 3.316666667               & 1.474293785                   \\ \hline
No visual & Personal & B & 60                         & 3.616666667               & 0.409887006                   \\ \hline
No visual & Personal & C & 60                         & 3                         & 2.13559322                    \\ \hline
Visual    & General  & A & 60                         & 2.983333333               & 1.30480226                    \\ \hline
Visual    & General  & B & 60                         & 3.55                      & 0.963559322                   \\ \hline
Visual    & General  & C & 60                         & 3.066666667               & 2.503954802                   \\ \hline
Visual    & Personal & A & 60                         & 3.883333333               & 0.816666667                   \\ \hline
Visual    & Personal & B & 60                         & 3.85                      & 0.638135593                   \\ \hline
Visual    & Personal & C & 60                         & 3.75                      & 0.597457627                   \\ \hline
          &          &   & 720                        & 3.377777778               & 1.297975583                   \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For likeability, having the visualisations had a slightly higher mean rating than without visualisations. Personalised stopping as opposed to general stops also had slightly higher ratings. Customer type B gave the highest ratings whilst the lowest ratings were given by customer type C.
\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\
\begin{table}[tb]
\caption{Intelligence}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
          &          &   & \multicolumn{1}{r|}{Count} & \multicolumn{1}{r|}{Mean} & \multicolumn{1}{r|}{Variance} \\ \hline
No visual &          &   & 300                        & 2.933333333               & 1.34671126                    \\ \hline
Visual    &          &   & 300                        & 3.303333333               & 1.255507246                   \\ \hline
          & General  &   & 300                        & 2.846666667               & 1.40115942                    \\ \hline
          & Personal &   & 300                        & 3.39                      & 1.121638796                   \\ \hline
          &          & A & 200                        & 3.085                     & 1.314346734                   \\ \hline
          &          & B & 200                        & 3.435                     & 0.819874372                   \\ \hline
          &          & C & 200                        & 2.835                     & 1.696256281                   \\ \hline
No visual & General  &   & 150                        & 2.826666667               & 1.352304251                   \\ \hline
No visual & Personal &   & 150                        & 3.04                      & 1.327248322                   \\ \hline
Visual    & General  &   & 150                        & 2.866666667               & 1.458612975                   \\ \hline
Visual    & Personal &   & 150                        & 3.74                      & 0.676912752                   \\ \hline
No visual &          & A & 100                        & 2.84                      & 1.408484848                   \\ \hline
No visual &          & B & 100                        & 3.39                      & 0.785757576                   \\ \hline
No visual &          & C & 100                        & 2.57                      & 1.52030303                    \\ \hline
Visual    &          & A & 100                        & 3.33                      & 1.112222222                   \\ \hline
Visual    &          & B & 100                        & 3.48                      & 0.858181818                   \\ \hline
Visual    &          & C & 100                        & 3.1                       & 1.747474747                   \\ \hline
          & General  & A & 100                        & 2.72                      & 1.052121212                   \\ \hline
          & General  & B & 100                        & 3.27                      & 0.946565657                   \\ \hline
          & General  & C & 100                        & 2.55                      & 1.946969697                   \\ \hline
          & Personal & A & 100                        & 3.45                      & 1.320707071                   \\ \hline
          & Personal & B & 100                        & 3.6                       & 0.646464646                   \\ \hline
          & Personal & C & 100                        & 3.12                      & 1.298585859                   \\ \hline
No visual & General  & A & 50                         & 2.58                      & 1.105714286                   \\ \hline
No visual & General  & B & 50                         & 3.44                      & 0.782040816                   \\ \hline
No visual & General  & C & 50                         & 2.46                      & 1.64122449                    \\ \hline
No visual & Personal & A & 50                         & 3.1                       & 1.602040816                   \\ \hline
No visual & Personal & B & 50                         & 3.34                      & 0.800408163                   \\ \hline
No visual & Personal & C & 50                         & 2.68                      & 1.405714286                   \\ \hline
Visual    & General  & A & 50                         & 2.86                      & 0.98                          \\ \hline
Visual    & General  & B & 50                         & 3.1                       & 1.071428571                   \\ \hline
Visual    & General  & C & 50                         & 2.64                      & 2.275918367                   \\ \hline
Visual    & Personal & A & 50                         & 3.8                       & 0.816326531                   \\ \hline
Visual    & Personal & B & 50                         & 3.86                      & 0.367755102                   \\ \hline
Visual    & Personal & C & 50                         & 3.56                      & 0.822857143                   \\ \hline
          &          &   & 600                        & 3.118333333               & 1.333219254                   \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For intelligence, having visualisations had a higher mean rating than without visualisations. Personalised stopping as opposed to general stops also had higher ratings. Customer type B gave the highest ratings whilst the lowest ratings were given by customer type C.
\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\
\begin{table}[tb]
\caption{Safety}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
          &          &   & \multicolumn{1}{r|}{Count} & \multicolumn{1}{r|}{Mean} & \multicolumn{1}{r|}{Variance} \\ \hline
No visual &          &   & 180                        & 3.194444444               & 1.397734327                   \\ \hline
Visual    &          &   & 180                        & 3.416666667               & 1.25                          \\ \hline
          & General  &   & 180                        & 3.216666667               & 1.410893855                   \\ \hline
          & Personal &   & 180                        & 3.394444444               & 1.245779019                   \\ \hline
          &          & A & 120                        & 3.475                     & 1.226260504                   \\ \hline
          &          & B & 120                        & 3.4                       & 1.115966387                   \\ \hline
          &          & C & 120                        & 3.041666667               & 1.569677871                   \\ \hline
No visual & General  &   & 90                         & 3.166666667               & 1.466292135                   \\ \hline
No visual & Personal &   & 90                         & 3.222222222               & 1.343320849                   \\ \hline
Visual    & General  &   & 90                         & 3.266666667               & 1.366292135                   \\ \hline
Visual    & Personal &   & 90                         & 3.566666667               & 1.102247191                   \\ \hline
No visual &          & A & 60                         & 3.433333333               & 1.232768362                   \\ \hline
No visual &          & B & 60                         & 3.3                       & 1.128813559                   \\ \hline
No visual &          & C & 60                         & 2.85                      & 1.688983051                   \\ \hline
Visual    &          & A & 60                         & 3.516666667               & 1.23700565                    \\ \hline
Visual    &          & B & 60                         & 3.5                       & 1.101694915                   \\ \hline
Visual    &          & C & 60                         & 3.233333333               & 1.402259887                   \\ \hline
          & General  & A & 60                         & 3.366666667               & 1.151412429                   \\ \hline
          & General  & B & 60                         & 3.316666667               & 1.135310734                   \\ \hline
          & General  & C & 60                         & 2.966666667               & 1.897175141                   \\ \hline
          & Personal & A & 60                         & 3.583333333               & 1.298022599                   \\ \hline
          & Personal & B & 60                         & 3.483333333               & 1.101412429                   \\ \hline
          & Personal & C & 60                         & 3.116666667               & 1.257344633                   \\ \hline
No visual & General  & A & 30                         & 3.266666667               & 1.167816092                   \\ \hline
No visual & General  & B & 30                         & 3.266666667               & 1.167816092                   \\ \hline
No visual & General  & C & 30                         & 2.966666667               & 2.102298851                   \\ \hline
No visual & Personal & A & 30                         & 3.6                       & 1.282758621                   \\ \hline
No visual & Personal & B & 30                         & 3.333333333               & 1.126436782                   \\ \hline
No visual & Personal & C & 30                         & 2.733333333               & 1.305747126                   \\ \hline
Visual    & General  & A & 30                         & 3.466666667               & 1.154022989                   \\ \hline
Visual    & General  & B & 30                         & 3.366666667               & 1.136781609                   \\ \hline
Visual    & General  & C & 30                         & 2.966666667               & 1.757471264                   \\ \hline
Visual    & Personal & A & 30                         & 3.566666667               & 1.357471264                   \\ \hline
Visual    & Personal & B & 30                         & 3.633333333               & 1.067816092                   \\ \hline
Visual    & Personal & C & 30                         & 3.5                       & 0.948275862                   \\ \hline
          &          &   & 360                        & 3.305555556               & 1.332559579                   \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For safety, having visualisations had a higher mean rating than without visualisations. Personalised stopping as opposed to general stops also had higher ratings. Customer type A gave the highest ratings whilst the lowest ratings were given by customer type C.
\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\
\begin{table}[tb]
\caption{Human-robot fluency}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
          &          &   & \multicolumn{1}{r|}{Count} & \multicolumn{1}{r|}{Mean} & \multicolumn{1}{r|}{Variance} \\ \hline
No visual &          &   & 120                        & 2.891666667               & 1.626820728                   \\ \hline
Visual    &          &   & 120                        & 3.433333333               & 1.592156863                   \\ \hline
          & General  &   & 120                        & 2.85                      & 1.725210084                   \\ \hline
          & Personal &   & 120                        & 3.475                     & 1.444747899                   \\ \hline
          &          & A & 80                         & 3.325                     & 1.462658228                   \\ \hline
          &          & B & 80                         & 3.475                     & 1.898101266                   \\ \hline
          &          & C & 80                         & 2.6875                    & 1.356803797                   \\ \hline
No visual & General  &   & 60                         & 2.783333333               & 1.596327684                   \\ \hline
No visual & Personal &   & 60                         & 3                         & 1.661016949                   \\ \hline
Visual    & General  &   & 60                         & 2.916666667               & 1.874293785                   \\ \hline
Visual    & Personal &   & 60                         & 3.95                      & 0.794067797                   \\ \hline
No visual &          & A & 40                         & 3.075                     & 1.507051282                   \\ \hline
No visual &          & B & 40                         & 3.05                      & 2.1                           \\ \hline
No visual &          & C & 40                         & 2.55                      & 1.176923077                   \\ \hline
Visual    &          & A & 40                         & 3.575                     & 1.327564103                   \\ \hline
Visual    &          & B & 40                         & 3.9                       & 1.374358974                   \\ \hline
Visual    &          & C & 40                         & 2.825                     & 1.532692308                   \\ \hline
          & General  & A & 40                         & 3                         & 1.282051282                   \\ \hline
          & General  & B & 40                         & 3.275                     & 2.204487179                   \\ \hline
          & General  & C & 40                         & 2.275                     & 1.230128205                   \\ \hline
          & Personal & A & 40                         & 3.65                      & 1.464102564                   \\ \hline
          & Personal & B & 40                         & 3.675                     & 1.558333333                   \\ \hline
          & Personal & C & 40                         & 3.1                       & 1.169230769                   \\ \hline
No visual & General  & A & 20                         & 2.95                      & 1.207894737                   \\ \hline
No visual & General  & B & 20                         & 3.05                      & 2.365789474                   \\ \hline
No visual & General  & C & 20                         & 2.35                      & 1.081578947                   \\ \hline
No visual & Personal & A & 20                         & 3.2                       & 1.852631579                   \\ \hline
No visual & Personal & B & 20                         & 3.05                      & 1.944736842                   \\ \hline
No visual & Personal & C & 20                         & 2.75                      & 1.25                          \\ \hline
Visual    & General  & A & 20                         & 3.05                      & 1.418421053                   \\ \hline
Visual    & General  & B & 20                         & 3.5                       & 2.052631579                   \\ \hline
Visual    & General  & C & 20                         & 2.2                       & 1.431578947                   \\ \hline
Visual    & Personal & A & 20                         & 4.1                       & 0.726315789                   \\ \hline
Visual    & Personal & B & 20                         & 4.3                       & 0.431578947                   \\ \hline
Visual    & Personal & C & 20                         & 3.45                      & 0.892105263                   \\ \hline
          &          &   & 240                        & 3.1625                    & 1.676412134                   \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For human-robot fluency, having visualisations had a higher mean rating than without visualisations. Personalised stopping as opposed to general stops also had higher ratings. Customer type B gave the highest ratings whilst the lowest ratings were given by customer type C.
\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\
\begin{table}[tb]
\caption{Trust in robot}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
          &          &   & \multicolumn{1}{r|}{Count} & \multicolumn{1}{r|}{Mean} & \multicolumn{1}{r|}{Variance} \\ \hline
No visual &          &   & 120                        & 2.858333333               & 1.467156863                   \\ \hline
Visual    &          &   & 120                        & 3.516666667               & 1.495518207                   \\ \hline
          & General  &   & 120                        & 3.025                     & 1.772478992                   \\ \hline
          & Personal &   & 120                        & 3.35                      & 1.355462185                   \\ \hline
          &          & A & 80                         & 3.2875                    & 1.549208861                   \\ \hline
          &          & B & 80                         & 3.55                      & 1.465822785                   \\ \hline
          &          & C & 80                         & 2.725                     & 1.417088608                   \\ \hline
No visual & General  &   & 60                         & 2.783333333               & 1.494632768                   \\ \hline
No visual & Personal &   & 60                         & 2.933333333               & 1.453107345                   \\ \hline
Visual    & General  &   & 60                         & 3.266666667               & 1.961581921                   \\ \hline
Visual    & Personal &   & 60                         & 3.766666667               & 0.927683616                   \\ \hline
No visual &          & A & 40                         & 2.825                     & 1.276282051                   \\ \hline
No visual &          & B & 40                         & 3.35                      & 1.669230769                   \\ \hline
No visual &          & C & 40                         & 2.4                       & 1.066666667                   \\ \hline
Visual    &          & A & 40                         & 3.75                      & 1.423076923                   \\ \hline
Visual    &          & B & 40                         & 3.75                      & 1.217948718                   \\ \hline
Visual    &          & C & 40                         & 3.05                      & 1.587179487                   \\ \hline
          & General  & A & 40                         & 3.25                      & 1.525641026                   \\ \hline
          & General  & B & 40                         & 3.375                     & 1.778846154                   \\ \hline
          & General  & C & 40                         & 2.45                      & 1.587179487                   \\ \hline
          & Personal & A & 40                         & 3.325                     & 1.609615385                   \\ \hline
          & Personal & B & 40                         & 3.725                     & 1.127564103                   \\ \hline
          & Personal & C & 40                         & 3                         & 1.128205128                   \\ \hline
No visual & General  & A & 20                         & 2.8                       & 1.010526316                   \\ \hline
No visual & General  & B & 20                         & 3.35                      & 2.028947368                   \\ \hline
No visual & General  & C & 20                         & 2.2                       & 0.905263158                   \\ \hline
No visual & Personal & A & 20                         & 2.85                      & 1.607894737                   \\ \hline
No visual & Personal & B & 20                         & 3.35                      & 1.397368421                   \\ \hline
No visual & Personal & C & 20                         & 2.6                       & 1.2                           \\ \hline
Visual    & General  & A & 20                         & 3.7                       & 1.694736842                   \\ \hline
Visual    & General  & B & 20                         & 3.4                       & 1.621052632                   \\ \hline
Visual    & General  & C & 20                         & 2.7                       & 2.221052632                   \\ \hline
Visual    & Personal & A & 20                         & 3.8                       & 1.221052632                   \\ \hline
Visual    & Personal & B & 20                         & 4.1                       & 0.621052632                   \\ \hline
Visual    & Personal & C & 20                         & 3.4                       & 0.778947368                   \\ \hline
          &          &   & 240                        & 3.1875                    & 1.583943515                   \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For trust in robot, having visualisations had a higher mean rating than without visualisations. Personalised stopping as opposed to general stops also had higher ratings. Customer type B gave the highest ratings whilst the lowest ratings were given by customer type C.
\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\

\begin{table}[tb]
\caption{Working Alliance}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
          &          &   & \multicolumn{1}{r|}{Count} & \multicolumn{1}{r|}{Mean} & \multicolumn{1}{r|}{Variance} \\ \hline
No visual &          &   & 180                        & 2.944444444               & 1.549968963                   \\ \hline
Visual    &          &   & 180                        & 3.616666667               & 1.612011173                   \\ \hline
          & General  &   & 180                        & 3.105555556               & 1.7597455                     \\ \hline
          & Personal &   & 180                        & 3.455555556               & 1.567846058                   \\ \hline
          &          & A & 120                        & 3.358333333               & 1.677240896                   \\ \hline
          &          & B & 120                        & 3.566666667               & 1.608963585                   \\ \hline
          &          & C & 120                        & 2.916666667               & 1.589635854                   \\ \hline
No visual & General  &   & 90                         & 3.044444444               & 1.526092385                   \\ \hline
No visual & Personal &   & 90                         & 2.844444444               & 1.571036205                   \\ \hline
Visual    & General  &   & 90                         & 3.166666667               & 2.005617978                   \\ \hline
Visual    & Personal &   & 90                         & 4.066666667               & 0.826966292                   \\ \hline
No visual &          & A & 60                         & 3.066666667               & 1.48700565                    \\ \hline
No visual &          & B & 60                         & 3.216666667               & 1.698022599                   \\ \hline
No visual &          & C & 60                         & 2.55                      & 1.268644068                   \\ \hline
Visual    &          & A & 60                         & 3.65                      & 1.722881356                   \\ \hline
Visual    &          & B & 60                         & 3.916666667               & 1.298022599                   \\ \hline
Visual    &          & C & 60                         & 3.283333333               & 1.664124294                   \\ \hline
          & General  & A & 60                         & 3.083333333               & 1.56920904                    \\ \hline
          & General  & B & 60                         & 3.616666667               & 1.426836158                   \\ \hline
          & General  & C & 60                         & 2.616666667               & 1.833615819                   \\ \hline
          & Personal & A & 60                         & 3.633333333               & 1.659887006                   \\ \hline
          & Personal & B & 60                         & 3.516666667               & 1.813276836                   \\ \hline
          & Personal & C & 60                         & 3.216666667               & 1.189548023                   \\ \hline
No visual & General  & A & 30                         & 3                         & 1.310344828                   \\ \hline
No visual & General  & B & 30                         & 3.766666667               & 1.012643678                   \\ \hline
No visual & General  & C & 30                         & 2.366666667               & 1.343678161                   \\ \hline
No visual & Personal & A & 30                         & 3.133333333               & 1.705747126                   \\ \hline
No visual & Personal & B & 30                         & 2.666666667               & 1.816091954                   \\ \hline
No visual & Personal & C & 30                         & 2.733333333               & 1.167816092                   \\ \hline
Visual    & General  & A & 30                         & 3.166666667               & 1.867816092                   \\ \hline
Visual    & General  & B & 30                         & 3.466666667               & 1.843678161                   \\ \hline
Visual    & General  & C & 30                         & 2.866666667               & 2.257471264                   \\ \hline
Visual    & Personal & A & 30                         & 4.133333333               & 1.154022989                   \\ \hline
Visual    & Personal & B & 30                         & 4.366666667               & 0.37816092                    \\ \hline
Visual    & Personal & C & 30                         & 3.7                       & 0.768965517                   \\ \hline
          &          &   & 360                        & 3.280555556               & 1.689871557                   \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For working alliance, having visualisations had a higher mean rating than without visualisations. Personalised stopping as opposed to general stops also had higher ratings. Customer type B gave the highest ratings whilst the lowest ratings were given by customer type C.
\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\
\begin{table}[tb]
\caption{Collaborativeness Total}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
          &          &   & \multicolumn{1}{r|}{Count} & \multicolumn{1}{r|}{Mean} & \multicolumn{1}{r|}{Variance} \\ \hline
No visual &          &   & 420                        & 2.904761905               & 1.542220707                   \\ \hline
Visual    &          &   & 420                        & 3.535714286               & 1.571513808                   \\ \hline
          & General  &   & 420                        & 3.00952381                & 1.756472326                   \\ \hline
          & Personal &   & 420                        & 3.430952381               & 1.467774747                   \\ \hline
          &          & A & 280                        & 3.328571429               & 1.569073221                   \\ \hline
          &          & B & 280                        & 3.535714286               & 1.640296979                   \\ \hline
          &          & C & 280                        & 2.796428571               & 1.474539171                   \\ \hline
No visual & General  &   & 210                        & 2.895238095               & 1.539211666                   \\ \hline
No visual & Personal &   & 210                        & 2.914285714               & 1.552426521                   \\ \hline
Visual    & General  &   & 210                        & 3.123809524               & 1.955889724                   \\ \hline
Visual    & Personal &   & 210                        & 3.947619048               & 0.853702438                   \\ \hline
No visual &          & A & 140                        & 3                         & 1.424460432                   \\ \hline
No visual &          & B & 140                        & 3.207142857               & 1.791315519                   \\ \hline
No visual &          & C & 140                        & 2.507142857               & 1.172610483                   \\ \hline
Visual    &          & A & 140                        & 3.657142857               & 1.507502569                   \\ \hline
Visual    &          & B & 140                        & 3.864285714               & 1.2836074                     \\ \hline
Visual    &          & C & 140                        & 3.085714286               & 1.618499486                   \\ \hline
          & General  & A & 140                        & 3.107142857               & 1.463257965                   \\ \hline
          & General  & B & 140                        & 3.45                      & 1.745683453                   \\ \hline
          & General  & C & 140                        & 2.471428571               & 1.589105858                   \\ \hline
          & Personal & A & 140                        & 3.55                      & 1.587410072                   \\ \hline
          & Personal & B & 140                        & 3.621428571               & 1.531911614                   \\ \hline
          & Personal & C & 140                        & 3.121428571               & 1.157810894                   \\ \hline
No visual & General  & A & 70                         & 2.928571429               & 1.16873706                    \\ \hline
No visual & General  & B & 70                         & 3.442857143               & 1.728571429                   \\ \hline
No visual & General  & C & 70                         & 2.314285714               & 1.117184265                   \\ \hline
No visual & Personal & A & 70                         & 3.071428571               & 1.69047619                    \\ \hline
No visual & Personal & B & 70                         & 2.971428571               & 1.767287785                   \\ \hline
No visual & Personal & C & 70                         & 2.7                       & 1.169565217                   \\ \hline
Visual    & General  & A & 70                         & 3.285714286               & 1.714285714                   \\ \hline
Visual    & General  & B & 70                         & 3.457142857               & 1.787991718                   \\ \hline
Visual    & General  & C & 70                         & 2.628571429               & 2.033954451                   \\ \hline
Visual    & Personal & A & 70                         & 4.028571429               & 1.042650104                   \\ \hline
Visual    & Personal & B & 70                         & 4.271428571               & 0.461490683                   \\ \hline
Visual    & Personal & C & 70                         & 3.542857143               & 0.802484472                   \\ \hline
          &          &   & 840                        & 3.220238095               & 1.654655486                   \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For total collaborativeness, having visualisations had a higher mean rating than without visualisations. Personalised stopping as opposed to general stops also had higher ratings. Customer type B gave the highest ratings whilst the lowest ratings were given by customer type C.
\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\
\begin{table}[tb]
\caption{Accuracy}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
          &          &   & \multicolumn{1}{r|}{Count} & \multicolumn{1}{r|}{Mean} & \multicolumn{1}{r|}{Variance} \\ \hline
No visual &          &   & 60                         & 35\%                      & 23\%                          \\ \hline
Visual    &          &   & 60                         & 72\%                      & 21\%                          \\ \hline
          & General  &   & 60                         & 47\%                      & 25\%                          \\ \hline
          & Personal &   & 60                         & 60\%                      & 24\%                          \\ \hline
          &          & A & 40                         & 48\%                      & 26\%                          \\ \hline
          &          & B & 40                         & 63\%                      & 24\%                          \\ \hline
          &          & C & 40                         & 50\%                      & 26\%                          \\ \hline
No visual & General  &   & 30                         & 37\%                      & 24\%                          \\ \hline
No visual & Personal &   & 30                         & 33\%                      & 23\%                          \\ \hline
Visual    & General  &   & 30                         & 57\%                      & 25\%                          \\ \hline
Visual    & Personal &   & 30                         & 87\%                      & 12\%                          \\ \hline
No visual &          & A & 20                         & 20\%                      & 17\%                          \\ \hline
No visual &          & B & 20                         & 55\%                      & 26\%                          \\ \hline
No visual &          & C & 20                         & 30\%                      & 22\%                          \\ \hline
Visual    &          & A & 20                         & 75\%                      & 20\%                          \\ \hline
Visual    &          & B & 20                         & 70\%                      & 22\%                          \\ \hline
Visual    &          & C & 20                         & 70\%                      & 22\%                          \\ \hline
          & General  & A & 20                         & 35\%                      & 24\%                          \\ \hline
          & General  & B & 20                         & 70\%                      & 22\%                          \\ \hline
          & General  & C & 20                         & 35\%                      & 24\%                          \\ \hline
          & Personal & A & 20                         & 60\%                      & 25\%                          \\ \hline
          & Personal & B & 20                         & 55\%                      & 26\%                          \\ \hline
          & Personal & C & 20                         & 65\%                      & 24\%                          \\ \hline
No visual & General  & A & 10                         & 20\%                      & 18\%                          \\ \hline
No visual & General  & B & 10                         & 80\%                      & 18\%                          \\ \hline
No visual & General  & C & 10                         & 10\%                      & 10\%                          \\ \hline
No visual & Personal & A & 10                         & 20\%                      & 18\%                          \\ \hline
No visual & Personal & B & 10                         & 30\%                      & 23\%                          \\ \hline
No visual & Personal & C & 10                         & 50\%                      & 28\%                          \\ \hline
Visual    & General  & A & 10                         & 50\%                      & 28\%                          \\ \hline
Visual    & General  & B & 10                         & 60\%                      & 27\%                          \\ \hline
Visual    & General  & C & 10                         & 60\%                      & 27\%                          \\ \hline
Visual    & Personal & A & 10                         & 100\%                     & 0\%                           \\ \hline
Visual    & Personal & B & 10                         & 80\%                      & 18\%                          \\ \hline
Visual    & Personal & C & 10                         & 80\%                      & 18\%                          \\ \hline
          &          &   & 120                        & 53\%                      & 25\%                          \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For accuracy, having visualisations had a significantly higher accuracy than without visualisations. Personalised stopping as opposed to general stops also had a higher accuracy. Customer type B had the highest accuracy whilst customer type A had the lowest accuracy.dd

\begin{table}[tb]
\caption{Perceived satisfaction}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
          &          &   & \multicolumn{1}{r|}{Count} & \multicolumn{1}{r|}{Mean} & \multicolumn{1}{r|}{Variance} \\ \hline
No visual &          &   & 60                         & 2.916666667               & 1.63700565                    \\ \hline
Visual    &          &   & 60                         & 3.383333333               & 1.359039548                   \\ \hline
          & General  &   & 60                         & 2.766666667               & 1.402259887                   \\ \hline
          & Personal &   & 60                         & 3.533333333               & 1.405649718                   \\ \hline
          &          & A & 40                         & 3.325                     & 1.507051282                   \\ \hline
          &          & B & 40                         & 3.275                     & 1.281410256                   \\ \hline
          &          & C & 40                         & 2.85                      & 1.771794872                   \\ \hline
No visual & General  &   & 30                         & 2.7                       & 1.527586207                   \\ \hline
No visual & Personal &   & 30                         & 3.133333333               & 1.705747126                   \\ \hline
Visual    & General  &   & 30                         & 2.833333333               & 1.316091954                   \\ \hline
Visual    & Personal &   & 30                         & 3.933333333               & 0.822988506                   \\ \hline
No visual &          & A & 20                         & 3.15                      & 1.397368421                   \\ \hline
No visual &          & B & 20                         & 3.05                      & 1.313157895                   \\ \hline
No visual &          & C & 20                         & 2.55                      & 2.155263158                   \\ \hline
Visual    &          & A & 20                         & 3.5                       & 1.631578947                   \\ \hline
Visual    &          & B & 20                         & 3.5                       & 1.210526316                   \\ \hline
Visual    &          & C & 20                         & 3.15                      & 1.292105263                   \\ \hline
          & General  & A & 20                         & 2.8                       & 1.431578947                   \\ \hline
          & General  & B & 20                         & 3                         & 1.263157895                   \\ \hline
          & General  & C & 20                         & 2.5                       & 1.526315789                   \\ \hline
          & Personal & A & 20                         & 3.85                      & 1.081578947                   \\ \hline
          & Personal & B & 20                         & 3.55                      & 1.207894737                   \\ \hline
          & Personal & C & 20                         & 3.2                       & 1.852631579                   \\ \hline
No visual & General  & A & 10                         & 2.8                       & 1.511111111                   \\ \hline
No visual & General  & B & 10                         & 3.1                       & 1.433333333                   \\ \hline
No visual & General  & C & 10                         & 2.2                       & 1.511111111                   \\ \hline
No visual & Personal & A & 10                         & 3.5                       & 1.166666667                   \\ \hline
No visual & Personal & B & 10                         & 3                         & 1.333333333                   \\ \hline
No visual & Personal & C & 10                         & 2.9                       & 2.766666667                   \\ \hline
Visual    & General  & A & 10                         & 2.8                       & 1.511111111                   \\ \hline
Visual    & General  & B & 10                         & 2.9                       & 1.211111111                   \\ \hline
Visual    & General  & C & 10                         & 2.8                       & 1.511111111                   \\ \hline
Visual    & Personal & A & 10                         & 4.2                       & 0.844444444                   \\ \hline
Visual    & Personal & B & 10                         & 4.1                       & 0.544444444                   \\ \hline
Visual    & Personal & C & 10                         & 3.5                       & 0.944444444                   \\ \hline
          &          &   & 120                        & 3.15                      & 1.540336134                   \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For perceived satisfaction, having visualisations had higher ratings than without visualisations. Personalised stopping as opposed to general stops also had higher ratings. Customer type A had the highest ratings whilst customer type C had the lowest ratings.
\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\
\begin{table}[tb]
\caption{Perceived quickness}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
          &          &   & \multicolumn{1}{r|}{Count} & \multicolumn{1}{r|}{Mean} & \multicolumn{1}{r|}{Variance} \\ \hline
No visual &          &   & 60                         & 3.75                      & 1.343220339                   \\ \hline
Visual    &          &   & 60                         & 3.333333333               & 1.005649718                   \\ \hline
          & General  &   & 60                         & 3.483333333               & 1.23700565                    \\ \hline
          & Personal &   & 60                         & 3.6                       & 1.193220339                   \\ \hline
          &          & A & 40                         & 3.575                     & 0.81474359                    \\ \hline
          &          & B & 40                         & 3.925                     & 0.840384615                   \\ \hline
          &          & C & 40                         & 3.125                     & 1.701923077                   \\ \hline
No visual & General  &   & 30                         & 3.766666667               & 1.426436782                   \\ \hline
No visual & Personal &   & 30                         & 3.733333333               & 1.305747126                   \\ \hline
Visual    & General  &   & 30                         & 3.2                       & 0.924137931                   \\ \hline
Visual    & Personal &   & 30                         & 3.466666667               & 1.085057471                   \\ \hline
No visual &          & A & 20                         & 3.7                       & 0.957894737                   \\ \hline
No visual &          & B & 20                         & 4.4                       & 0.357894737                   \\ \hline
No visual &          & C & 20                         & 3.15                      & 2.028947368                   \\ \hline
Visual    &          & A & 20                         & 3.45                      & 0.681578947                   \\ \hline
Visual    &          & B & 20                         & 3.45                      & 0.892105263                   \\ \hline
Visual    &          & C & 20                         & 3.1                       & 1.463157895                   \\ \hline
          & General  & A & 20                         & 3.5                       & 0.894736842                   \\ \hline
          & General  & B & 20                         & 3.9                       & 0.831578947                   \\ \hline
          & General  & C & 20                         & 3.05                      & 1.734210526                   \\ \hline
          & Personal & A & 20                         & 3.65                      & 0.765789474                   \\ \hline
          & Personal & B & 20                         & 3.95                      & 0.892105263                   \\ \hline
          & Personal & C & 20                         & 3.2                       & 1.747368421                   \\ \hline
No visual & General  & A & 10                         & 3.6                       & 1.155555556                   \\ \hline
No visual & General  & B & 10                         & 4.5                       & 0.277777778                   \\ \hline
No visual & General  & C & 10                         & 3.2                       & 2.177777778                   \\ \hline
No visual & Personal & A & 10                         & 3.8                       & 0.844444444                   \\ \hline
No visual & Personal & B & 10                         & 4.3                       & 0.455555556                   \\ \hline
No visual & Personal & C & 10                         & 3.1                       & 2.1                           \\ \hline
Visual    & General  & A & 10                         & 3.4                       & 0.711111111                   \\ \hline
Visual    & General  & B & 10                         & 3.3                       & 0.677777778                   \\ \hline
Visual    & General  & C & 10                         & 2.9                       & 1.433333333                   \\ \hline
Visual    & Personal & A & 10                         & 3.5                       & 0.722222222                   \\ \hline
Visual    & Personal & B & 10                         & 3.6                       & 1.155555556                   \\ \hline
Visual    & Personal & C & 10                         & 3.3                       & 1.566666667                   \\ \hline
          &          &   & 120                        & 3.541666667               & 1.208333333                   \\ \hline
          &          &   &                            &                           &                               \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For perceived satisfaction, having visualisations had lower ratings than without visualisations. Personalised stopping as opposed to general stops had higher ratings. Customer type B had the highest ratings whilst customer type C had the lowest ratings.


\subsection{Three Factor ANOVAs}
\begin{table}[tb]
\caption{Anthropomorphism}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Three   Way Anova \\      (via Regression)\end{tabular}                    &                                  &                                  &                                  & \multicolumn{1}{c|}{Alpha}      & \multicolumn{1}{c|}{0.05}             &                                        \\ \hline
\multicolumn{1}{|c|}{\textit{}}                                                                       & \multicolumn{1}{c|}{\textit{SS}} & \multicolumn{1}{c|}{\textit{df}} & \multicolumn{1}{c|}{\textit{MS}} & \multicolumn{1}{c|}{\textit{F}} & \multicolumn{1}{c|}{\textit{p-value}} & \multicolumn{1}{c|}{\textit{p eta-sq}} \\ \hline
Indications                                                                                           & 9.126666667                      & 1                                & 9.126666667                      & 7.366276835                     & 0.006840798                           & 0.01237                                \\ \hline
Stopping type                                                                                         & 3.84                             & 1                                & 3.84                             & 3.099324658                     & 0.078844614                           & 0.00524                                \\ \hline
Customer type                                                                                         & 22.14333333                      & 2                                & 11.07166667                      & 8.936117059                     & 0.000150281                           & 0.0295                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type\end{tabular}                         & 5.226666667                      & 1                                & 5.226666667                      & 4.218525229                     & 0.040426509                           & 0.00712                                \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Customer type\end{tabular}                         & 1.463333333                      & 2                                & 0.731666667                      & 0.590539724                     & 0.442519009                           & 0.002                                  \\ \hline
\begin{tabular}[c]{@{}l@{}}Stopping   type \\      x Customer type\end{tabular}                       & 8.71                             & 2                                & 4.355                            & 3.514989293                     & 0.030374765                           & 0.01181                                \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type \\      x Customer type\end{tabular} & 0.963333333                      & 2                                & 0.481666667                      & 0.388760775                     & 0.67807053                            & 0.00132                                \\ \hline
Within                                                                                                & 728.52                           & 588                              & 1.238979592                      &                                 &                                       &                                        \\ \hline
Total                                                                                                 & 779.9933333                      & 599                              & 1.302159154                      &                                 &                                       &                                        \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For anthropomorphism, the presence of indications, stopping type and customer type was statistically significant, as well as the joint significance of indications with stopping type and stopping type with customer type. The rest of the joint combinations were not statistically significant.
\begin{table}[tb]
\caption{Animacy}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Three   Way Anova \\      (via Regression)\end{tabular}                    &                                  &                                  &                                  & \multicolumn{1}{c|}{Alpha}      & \multicolumn{1}{c|}{0.05}             &                                        \\ \hline
\multicolumn{1}{|c|}{\textit{}}                                                                       & \multicolumn{1}{c|}{\textit{SS}} & \multicolumn{1}{c|}{\textit{df}} & \multicolumn{1}{c|}{\textit{MS}} & \multicolumn{1}{c|}{\textit{F}} & \multicolumn{1}{c|}{\textit{p-value}} & \multicolumn{1}{c|}{\textit{p eta-sq}} \\ \hline
Indications                                                                                           & 1.601666667                      & 1                                & 1.601666667                      & 1.405935569                     & 0.23621122                            & 0.00239                                \\ \hline
Stopping type                                                                                         & 12.615                           & 1                                & 12.615                           & 11.07338847                     & 0.000930445                           & 0.01848                                \\ \hline
Customer type                                                                                         & 20.66333333                      & 2                                & 10.33166667                      & 9.069089063                     & 0.000132091                           & 0.02992                                \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type\end{tabular}                         & 6.201666667                      & 1                                & 6.201666667                      & 5.443794226                     & 0.019974214                           & 0.00917                                \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Customer type\end{tabular}                         & 1.323333333                      & 2                                & 0.661666667                      & 0.58080793                      & 0.446301394                           & 0.00197                                \\ \hline
\begin{tabular}[c]{@{}l@{}}Stopping   type \\      x Customer type\end{tabular}                       & 10.21                            & 2                                & 5.105                            & 4.481145314                     & 0.011709701                           & 0.01501                                \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type \\      x Customer type\end{tabular} & 2.123333333                      & 2                                & 1.061666667                      & 0.931926074                     & 0.394375345                           & 0.00316                                \\ \hline
Within                                                                                                & 669.86                           & 588                              & 1.139217687                      &                                 &                                       &                                        \\ \hline
Total                                                                                                 & 724.5983333                      & 599                              & 1.209680022                      &                                 &                                       &                                        \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For animacy, indications were not statistically significant whilst stopping type and customer type were. For the joint combinations, indications with stopping type as well as stopping type with customer type were statistically significant whilst the rest are not.

\begin{table}[tb]
\caption{Likeability}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Three   Way Anova \\      (via Regression)\end{tabular}                    &                                  &                                  &                                  & \multicolumn{1}{c|}{Alpha}      & \multicolumn{1}{c|}{0.05}             &                                        \\ \hline
\multicolumn{1}{|c|}{\textit{}}                                                                       & \multicolumn{1}{c|}{\textit{SS}} & \multicolumn{1}{c|}{\textit{df}} & \multicolumn{1}{c|}{\textit{MS}} & \multicolumn{1}{c|}{\textit{F}} & \multicolumn{1}{c|}{\textit{p-value}} & \multicolumn{1}{c|}{\textit{p eta-sq}} \\ \hline
Indications                                                                                           & 13.33888889                      & 1                                & 13.33888889                      & 11.26468132                     & 0.000832146                           & 0.015661385                            \\ \hline
Stopping type                                                                                         & 26.45                            & 1                                & 26.45                            & 22.33700449                     & 2.76024E-06                           & 0.030584517                            \\ \hline
Customer type                                                                                         & 32.01111111                      & 2                                & 16.00555556                      & 13.51667926                     & 1.73411E-06                           & 0.03677841                             \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type\end{tabular}                         & 10.75555556                      & 1                                & 10.75555556                      & 9.083058328                     & 0.002671988                           & 0.012666675                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Customer type\end{tabular}                         & 5.911111111                      & 2                                & 2.955555556                      & 2.495964375                     & 0.114585074                           & 0.007001382                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Stopping   type \\      x Customer type\end{tabular}                       & 5.2                              & 2                                & 2.6                              & 2.195697984                     & 0.112038069                           & 0.006164302                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type \\      x Customer type\end{tabular} & 1.211111111                      & 2                                & 0.605555556                      & 0.511391197                     & 0.599882082                           & 0.001442524                            \\ \hline
Within                                                                                                & 838.3666667                      & 708                              & 1.18413371                       &                                 &                                       &                                        \\ \hline
Total                                                                                                 & 933.2444444                      & 719                              & 1.297975583                      &                                 &                                       &                                        \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For likeability, the presence of indications, stopping type and customer type was statistically significant, as well as the joint significance of indications with stopping type. The rest of the joint combinations were not statistically significant.
\begin{table}[tb]
\caption{Intelligence}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Three   Way Anova \\      (via Regression)\end{tabular}                    &                                  &                                  &                                  & \multicolumn{1}{c|}{Alpha}      & \multicolumn{1}{c|}{0.05}             &                                        \\ \hline
\multicolumn{1}{|c|}{\textit{}}                                                                       & \multicolumn{1}{c|}{\textit{SS}} & \multicolumn{1}{c|}{\textit{df}} & \multicolumn{1}{c|}{\textit{MS}} & \multicolumn{1}{c|}{\textit{F}} & \multicolumn{1}{c|}{\textit{p-value}} & \multicolumn{1}{c|}{\textit{p eta-sq}} \\ \hline
Indications                                                                                           & 20.535                           & 1                                & 20.535                           & 18.02445141                     & 2.53424E-05                           & 0.029742119                            \\ \hline
Stopping type                                                                                         & 44.28166667                      & 1                                & 44.28166667                      & 38.86792059                     & 8.66034E-10                           & 0.062003365                            \\ \hline
Customer type                                                                                         & 36.33333333                      & 2                                & 18.16666667                      & 15.94566353                     & 1.80368E-07                           & 0.051446642                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type\end{tabular}                         & 16.335                           & 1                                & 16.335                           & 14.33793103                     & 0.000168448                           & 0.023803799                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Customer type\end{tabular}                         & 5.92                             & 2                                & 2.96                             & 2.598119122                     & 0.107527211                           & 0.008759729                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Stopping   type \\      x Customer type\end{tabular}                       & 4.053333333                      & 2                                & 2.026666667                      & 1.778892372                     & 0.169732391                           & 0.006014264                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type \\      x Customer type\end{tabular} & 1.24                             & 2                                & 0.62                             & 0.544200627                     & 0.580597471                           & 0.001847603                            \\ \hline
Within                                                                                                & 669.9                            & 588                              & 1.139285714                      &                                 &                                       &                                        \\ \hline
Total                                                                                                 & 798.5983333                      & 599                              & 1.333219254                      &                                 &                                       &                                        \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For intelligence, the presence of indications, stopping type and customer type was statistically significant, as well as the joint significance of indications with stopping type. The other joint combinations were not statistically significant.


\begin{table}[tb]
\caption{Safety}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Three   Way Anova \\      (via Regression)\end{tabular}                    &                                  &                                  &                                  & \multicolumn{1}{c|}{Alpha}      & \multicolumn{1}{c|}{0.05}             &                                        \\ \hline
\multicolumn{1}{|c|}{\textit{}}                                                                       & \multicolumn{1}{c|}{\textit{SS}} & \multicolumn{1}{c|}{\textit{df}} & \multicolumn{1}{c|}{\textit{MS}} & \multicolumn{1}{c|}{\textit{F}} & \multicolumn{1}{c|}{\textit{p-value}} & \multicolumn{1}{c|}{\textit{p eta-sq}} \\ \hline
Indications                                                                                           & 4.444444444                      & 1                                & 4.444444444                      & 3.424354244                     & 0.065088711                           & 0.009744214                            \\ \hline
Stopping type                                                                                         & 2.844444444                      & 1                                & 2.844444444                      & 2.191586716                     & 0.13967105                            & 0.006258251                            \\ \hline
Customer type                                                                                         & 12.87222222                      & 2                                & 6.436111111                      & 4.958892989                     & 0.007524847                           & 0.027709676                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type\end{tabular}                         & 1.344444444                      & 1                                & 1.344444444                      & 1.035867159                     & 0.309491664                           & 0.002967796                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Customer type\end{tabular}                         & 1.372222222                      & 2                                & 0.686111111                      & 0.528634686                     & 0.46767025                            & 0.003028928                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Stopping   type \\      x Customer type\end{tabular}                       & 0.072222222                      & 2                                & 0.036111111                      & 0.027822878                     & 0.972562776                           & 0.000159876                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type \\      x Customer type\end{tabular} & 3.772222222                      & 2                                & 1.886111111                      & 1.453210332                     & 0.235233778                           & 0.008282609                            \\ \hline
Within                                                                                                & 451.6666667                      & 348                              & 1.29789272                       &                                 &                                       &                                        \\ \hline
Total                                                                                                 & 478.3888889                      & 359                              & 1.332559579                      &                                 &                                       &                                        \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For safety, only indications and customer type were statistically significant while stopping type and all the combinations of the variables were not statistically significant.
\begin{table}[tb]
\caption{Human-robot fluency}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Three   Way Anova \\      (via Regression)\end{tabular}                    &                                  &                                  &                                  & \multicolumn{1}{c|}{Alpha}      & \multicolumn{1}{c|}{0.05}             &                                        \\ \hline
\multicolumn{1}{|c|}{\textit{}}                                                                       & \multicolumn{1}{c|}{\textit{SS}} & \multicolumn{1}{c|}{\textit{df}} & \multicolumn{1}{c|}{\textit{MS}} & \multicolumn{1}{c|}{\textit{F}} & \multicolumn{1}{c|}{\textit{p-value}} & \multicolumn{1}{c|}{\textit{p eta-sq}} \\ \hline
Indications                                                                                           & 17.60416667                      & 1                                & 17.60416667                      & 12.68367831                     & 0.000448966                           & 0.052698539                            \\ \hline
Stopping type                                                                                         & 23.4375                          & 1                                & 23.4375                          & 16.88655396                     & 5.53634E-05                           & 0.06895664                             \\ \hline
Customer type                                                                                         & 27.975                           & 2                                & 13.9875                          & 10.0778954                      & 6.39719E-05                           & 0.081222327                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type\end{tabular}                         & 10.00416667                      & 1                                & 10.00416667                      & 7.207931743                     & 0.007791257                           & 0.030644935                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Customer type\end{tabular}                         & 3.358333333                      & 2                                & 1.679166667                      & 1.209827777                     & 0.272526217                           & 0.010501081                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Stopping   type \\      x Customer type\end{tabular}                       & 1.825                            & 2                                & 0.9125                           & 0.657449834                     & 0.519150581                           & 0.005734035                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type \\      x Customer type\end{tabular} & 0.008333333                      & 2                                & 0.004166667                      & 0.003002054                     & 0.997002487                           & 2.63331E-05                            \\ \hline
Within                                                                                                & 316.45                           & 228                              & 1.387938596                      &                                 &                                       &                                        \\ \hline
Total                                                                                                 & 400.6625                         & 239                              & 1.676412134                      &                                 &                                       &                                        \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For human-robot fluency, the presence of indications, stopping type and customer type was statistically significant, as well as the joint significance of indications with stopping type. The rest of the joint combinations were not statistically significant.

\begin{table}[tb]
\caption{Trust in robot}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Three   Way Anova \\      (via Regression)\end{tabular}                    &                                  &                                  &                                  & \multicolumn{1}{c|}{Alpha}      & \multicolumn{1}{c|}{0.05}             &                                        \\ \hline
\multicolumn{1}{|c|}{\textit{}}                                                                       & \multicolumn{1}{c|}{\textit{SS}} & \multicolumn{1}{c|}{\textit{df}} & \multicolumn{1}{c|}{\textit{MS}} & \multicolumn{1}{c|}{\textit{F}} & \multicolumn{1}{c|}{\textit{p-value}} & \multicolumn{1}{c|}{\textit{p eta-sq}} \\ \hline
Indications                                                                                           & 26.00416667                      & 1                                & 26.00416667                      & 19.13490399                     & 1.85345E-05                           & 0.077426959                            \\ \hline
Stopping type                                                                                         & 6.3375                           & 1                                & 6.3375                           & 4.663385509                     & 0.031855817                           & 0.020043487                            \\ \hline
Customer type                                                                                         & 28.425                           & 2                                & 14.2125                          & 10.4581249                      & 4.51338E-05                           & 0.084029266                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type\end{tabular}                         & 1.8375                           & 1                                & 1.8375                           & 1.352105858                     & 0.246125903                           & 0.005895328                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Customer type\end{tabular}                         & 2.758333333                      & 2                                & 1.379166667                      & 1.014845893                     & 0.314812621                           & 0.008823608                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Stopping   type \\      x Customer type\end{tabular}                       & 2.275                            & 2                                & 1.1375                           & 0.837017912                     & 0.434325916                           & 0.007288746                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type \\      x Customer type\end{tabular} & 1.075                            & 2                                & 0.5375                           & 0.395513958                     & 0.673794953                           & 0.003457425                            \\ \hline
Within                                                                                                & 309.85                           & 228                              & 1.358991228                      &                                 &                                       &                                        \\ \hline
Total                                                                                                 & 378.5625                         & 239                              & 1.583943515                      &                                 &                                       &                                        \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For trust in robot, indications, stopping type and customer type were statistically significant. However, all the combinations of the three variable were not statistically significant.
\begin{table}[tb]
\caption{Working alliance}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Three   Way Anova \\      (via Regression)\end{tabular}                    &                                  &                                  &                                  & \multicolumn{1}{c|}{Alpha}      & \multicolumn{1}{c|}{0.05}             &                                        \\ \hline
\multicolumn{1}{|c|}{\textit{}}                                                                       & \multicolumn{1}{c|}{\textit{SS}} & \multicolumn{1}{c|}{\textit{df}} & \multicolumn{1}{c|}{\textit{MS}} & \multicolumn{1}{c|}{\textit{F}} & \multicolumn{1}{c|}{\textit{p-value}} & \multicolumn{1}{c|}{\textit{p eta-sq}} \\ \hline
Indications                                                                                           & 40.66944444                      & 1                                & 40.66944444                      & 29.35285171                     & 1.12836E-07                           & 0.077786219                            \\ \hline
Stopping type                                                                                         & 11.025                           & 1                                & 11.025                           & 7.957207052                     & 0.005064328                           & 0.022354392                            \\ \hline
Customer type                                                                                         & 26.43888889                      & 2                                & 13.21944444                      & 9.541030073                     & 9.24695E-05                           & 0.051983091                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type\end{tabular}                         & 27.225                           & 1                                & 27.225                           & 19.64942966                     & 1.24866E-05                           & 0.053446104                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Customer type\end{tabular}                         & 0.372222222                      & 2                                & 0.186111111                      & 0.134324231                     & 0.714212723                           & 0.000771383                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Stopping   type \\      x Customer type\end{tabular}                       & 9.15                             & 2                                & 4.575                            & 3.301970273                     & 0.037967278                           & 0.018623427                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type \\      x Customer type\end{tabular} & 9.616666667                      & 2                                & 4.808333333                      & 3.470376772                     & 0.032186043                           & 0.019554682                            \\ \hline
Within                                                                                                & 482.1666667                      & 348                              & 1.385536398                      &                                 &                                       &                                        \\ \hline
Total                                                                                                 & 606.6638889                      & 359                              & 1.689871557                      &                                 &                                       &                                        \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For working alliance, all variables and well as the joint combinations, except the the combination of indications and customer type, were statistically significant.

\begin{table}[tb]
\caption{Collaborativeness total}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Three   Way Anova \\      (via Regression)\end{tabular}                    &                                  &                                  &                                  & \multicolumn{1}{c|}{Alpha}      & \multicolumn{1}{c|}{0.05}             &                                        \\ \hline
\multicolumn{1}{|c|}{\textit{}}                                                                       & \multicolumn{1}{c|}{\textit{SS}} & \multicolumn{1}{c|}{\textit{df}} & \multicolumn{1}{c|}{\textit{MS}} & \multicolumn{1}{c|}{\textit{F}} & \multicolumn{1}{c|}{\textit{p-value}} & \multicolumn{1}{c|}{\textit{p eta-sq}} \\ \hline
Indications                                                                                           & 83.60119048                      & 1                                & 83.60119048                      & 60.85737431                     & 1.84622E-14                           & 0.068466974                            \\ \hline
Stopping type                                                                                         & 37.29642857                      & 1                                & 37.29642857                      & 27.14988508                     & 2.37845E-07                           & 0.031748686                            \\ \hline
Customer type                                                                                         & 81.4452381                       & 2                                & 40.72261905                      & 29.64397584                     & 3.67928E-13                           & 0.066819291                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type\end{tabular}                         & 34.00119048                      & 1                                & 34.00119048                      & 24.75112094                     & 7.93443E-07                           & 0.029025023                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Customer type\end{tabular}                         & 0.288095238                      & 2                                & 0.144047619                      & 0.104859271                     & 0.74615623                            & 0.000253219                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Stopping   type \\      x Customer type\end{tabular}                       & 8.064285714                      & 2                                & 4.032142857                      & 2.935192977                     & 0.053673447                           & 0.007039926                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type \\      x Customer type\end{tabular} & 6.116666667                      & 2                                & 3.058333333                      & 2.226309642                     & 0.10857165                            & 0.005348796                            \\ \hline
Within                                                                                                & 1137.442857                      & 828                              & 1.373723257                      &                                 &                                       &                                        \\ \hline
Total                                                                                                 & 1388.255952                      & 839                              & 1.654655486                      &                                 &                                       &                                        \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For overall collaborativeness, the presence of indications, stopping type and customer type was statistically significant, as well as the joint significance of indications with stopping type. The rest of the joint combinations were not statistically significant.
\begin{table}[tb]
\caption{Accuracy}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Three   Way Anova \\      (via Regression)\end{tabular}                    &                                  &                                  &                                  & \multicolumn{1}{c|}{Alpha}      & \multicolumn{1}{c|}{0.05}             &                                        \\ \hline
\multicolumn{1}{|c|}{\textit{}}                                                                       & \multicolumn{1}{c|}{\textit{SS}} & \multicolumn{1}{c|}{\textit{df}} & \multicolumn{1}{c|}{\textit{MS}} & \multicolumn{1}{c|}{\textit{F}} & \multicolumn{1}{c|}{\textit{p-value}} & \multicolumn{1}{c|}{\textit{p eta-sq}} \\ \hline
Indications                                                                                           & 4.033333333                      & 1                                & 4.033333333                      & 20.94230769                     & 1.27061E-05                           & 0.162416107                            \\ \hline
Stopping type                                                                                         & 0.533333333                      & 1                                & 0.533333333                      & 2.769230769                     & 0.098991261                           & 0.025                                  \\ \hline
Customer type                                                                                         & 0.516666667                      & 2                                & 0.258333333                      & 1.341346154                     & 0.265814218                           & 0.024237686                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type\end{tabular}                         & 0.833333333                      & 1                                & 0.833333333                      & 4.326923077                     & 0.039880476                           & 0.038520801                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Customer type\end{tabular}                         & 0.816666667                      & 2                                & 0.408333333                      & 2.120192308                     & 0.148269244                           & 0.037779491                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Stopping   type \\      x Customer type\end{tabular}                       & 1.216666667                      & 2                                & 0.608333333                      & 3.158653846                     & 0.046433932                           & 0.055261166                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type \\      x Customer type\end{tabular} & 1.116666667                      & 2                                & 0.558333333                      & 2.899038462                     & 0.059374089                           & 0.05095057                             \\ \hline
Within                                                                                                & 20.8                             & 108                              & 0.192592593                      &                                 &                                       &                                        \\ \hline
Total                                                                                                 & 29.86666667                      & 119                              & 0.250980392                      &                                 &                                       &                                        \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For accuracy, the presence of indications was statistically significant, as well as the joint significance of indications with stopping type, and the joint significance of the stopping type and customer type. The other variables and joint combinations were not statistically significant.

\begin{table}[tb]
\caption{Perceived satisfaction}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Three   Way Anova \\      (via Regression)\end{tabular}                    &                                  &                                  &                                  & \multicolumn{1}{c|}{Alpha}      & \multicolumn{1}{c|}{0.05}             &                                        \\ \hline
\multicolumn{1}{|c|}{\textit{}}                                                                       & \multicolumn{1}{c|}{\textit{SS}} & \multicolumn{1}{c|}{\textit{df}} & \multicolumn{1}{c|}{\textit{MS}} & \multicolumn{1}{c|}{\textit{F}} & \multicolumn{1}{c|}{\textit{p-value}} & \multicolumn{1}{c|}{\textit{p eta-sq}} \\ \hline
Indications                                                                                           & 6.533333333                      & 1                                & 6.533333333                      & 4.813096862                     & 0.030387063                           & 0.042664345                            \\ \hline
Stopping type                                                                                         & 17.63333333                      & 1                                & 17.63333333                      & 12.9904502                      & 0.000475197                           & 0.107367566                            \\ \hline
Customer type                                                                                         & 5.45                             & 2                                & 2.725                            & 2.007503411                     & 0.139305247                           & 0.035843473                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type\end{tabular}                         & 3.333333333                      & 1                                & 3.333333333                      & 2.455661664                     & 0.120027232                           & 0.022232103                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Customer type\end{tabular}                         & 0.316666667                      & 2                                & 0.158333333                      & 0.116643929                     & 0.73336693                            & 0.002155417                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Stopping   type \\      x Customer type\end{tabular}                       & 1.316666667                      & 2                                & 0.658333333                      & 0.484993179                     & 0.617035831                           & 0.008901408                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type \\      x Customer type\end{tabular} & 2.116666667                      & 2                                & 1.058333333                      & 0.779672578                     & 0.461119721                           & 0.014232881                            \\ \hline
Within                                                                                                & 146.6                            & 108                              & 1.357407407                      &                                 &                                       &                                        \\ \hline
Total                                                                                                 & 183.3                            & 119                              & 1.540336134                      &                                 &                                       &                                        \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For perceived satisfaction, while indications and stopping type are statistically significant, customer type and the joint combination of these variables are not statistically significant.
\begin{table}[tb]
\caption{Perceived quickness}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Three   Way Anova \\      (via Regression)\end{tabular}                    &                                  &                                  &                                  & \multicolumn{1}{c|}{Alpha}      & \multicolumn{1}{c|}{0.05}             &                                        \\ \hline
\multicolumn{1}{|c|}{\textit{}}                                                                       & \multicolumn{1}{c|}{\textit{SS}} & \multicolumn{1}{c|}{\textit{df}} & \multicolumn{1}{c|}{\textit{MS}} & \multicolumn{1}{c|}{\textit{F}} & \multicolumn{1}{c|}{\textit{p-value}} & \multicolumn{1}{c|}{\textit{p eta-sq}} \\ \hline
Indications                                                                                           & 5.208333333                      & 1                                & 5.208333333                      & 4.707112971                     & 0.032230098                           & 0.041764116                            \\ \hline
Stopping type                                                                                         & 0.408333333                      & 1                                & 0.408333333                      & 0.369037657                     & 0.544804487                           & 0.003405379                            \\ \hline
Customer type                                                                                         & 12.86666667                      & 2                                & 6.433333333                      & 5.814225941                     & 0.003997797                           & 0.097204734                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type\end{tabular}                         & 0.675                            & 1                                & 0.675                            & 0.610041841                     & 0.436480776                           & 0.005616809                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Customer type\end{tabular}                         & 4.466666667                      & 2                                & 2.233333333                      & 2.018410042                     & 0.158282511                           & 0.036031191                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Stopping   type \\      x Customer type\end{tabular}                       & 0.066666667                      & 2                                & 0.033333333                      & 0.030125523                     & 0.970331879                           & 0.000557569                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Indications   \\      x Stopping type \\      x Customer type\end{tabular} & 0.6                              & 2                                & 0.3                              & 0.271129707                     & 0.763035046                           & 0.004995837                            \\ \hline
Within                                                                                                & 119.5                            & 108                              & 1.106481481                      &                                 &                                       &                                        \\ \hline
Total                                                                                                 & 143.7916667                      & 119                              & 1.208333333                      &                                 &                                       &                                        \\ \hline
\end{tabular}
\end{table}
\subsubsection{}
For perceived quickness, while indications and customer type were statistically significant, stopping type was not statistically significant as well as all the joining combinations of the variables.
